Registration of serial sections: An evaluation method based on distortions of the ground truths

Registration of histological serial sections is a challenging task. Serial sections exhibit distortions and damage from sectioning. Missing information on how the tissue looked before cutting makes a realistic validation of 2D registrations extremely difficult. This work proposes methods for ground-truth-based evaluation of registrations. Firstly, we present a methodology to generate test data for registrations. We distort an innately registered image stack in the manner similar to the cutting distortion of serial sections. Test cases are generated from existing 3D data sets, thus the ground truth is known. Secondly, our test case generation premises evaluation of the registrations with known ground truths. Our methodology for such an evaluation technique distinguishes this work from other approaches. Both under- and over-registration become evident in our evaluations. We also survey existing validation efforts. We present a full-series evaluation across six different registration methods applied to our distorted 3D data sets of animal lungs. Our distorted and ground truth data sets are made publicly available.

==> extracted.tex <==
%% notice, we already have our own prelude.tex where such things could appear
%% but it looks more fitting to have directly text-related things here
\newcommand{\elastix}{{elastix}\xspace}
\newcommand{\activecontour}{\textsf{activecontour}\xspace}
\newcommand{\mytimes}{\ensuremath{\mskip\medmuskip\times\mskip\medmuskip}}
\newcommand{\kroi}[2]{\textup{#1}\textit{k}$\mytimes$\textup{#2}\textit{k}~pixels}
\newcommand{\xroi}[2]{\textup{#1}$\mytimes$\textup{#2}~pixels}

\hypertarget{pair-wise-evaluation}{%
\subsection{Pair-wise evaluation}\label{pair-wise-evaluation}}

\begin{table}[tbh]
\centering
\caption{Numerical values for the evaluation of the registrations on the CT data set, in the middle of the series (Figs. \ref{fig:eval-ct-1}, \ref{fig:eval-ct-2}). In Jaccard measure, we used a global threshold of~100. Low values in blending transforms can be explained by residual shifts. Notice the differences between the rigid-only and non-rigid methods. Notice also the lower values in the ground truth, when compared to \elastix. The "Locally distorted" line shows the local distortions only, without global rigid transforms. There was some larger movement (as seen in Fig.~\ref{fig:eval-ct-2}), this fact affects the measures. The registrations' inputs, however, were also rigidly transformed beforehand.\newline%
The larger the values, the better---up to the ground truth value.}
%
%\tfcomment{For example, does Table1 correspond to Fig.6 ?
%I meant, is the score in Table 1 calculated from one image pair or from 599 adjacent pairs?
%If from 599 pairs, the error distribution will be more informative than the average.}
%\olcomment{it is from the middle, not all pairs}
%\olcomment{now fixed with a further section!}
%
\label{tab:eval-ct}
\begin{tabular}{r S[round-mode = figures, round-precision = 3, table-format = 1.3] S[round-mode = figures, round-precision = 3, table-format = 2.1] S[round-mode = figures, round-precision = 3, table-format = 1.3]}
\multicolumn{4}{c}{\emph{CT}} \\
\toprule
%Method       & Jaccard & PSNR & SSIM \\
\multicolumn{1}{c}{Method}       & {Jaccard} & {PSNR} & {SSIM} \\
\midrule
Rigid-SIFT   & 0.12618114772989167  & 22.2166 & 0.47626 \\
Rigid-SURF   & 0.1350185873605948   & 22.7097 & 0.50812 \\
Deform-SURF  & 0.3753199268738574   & 28.5062 & 0.77221 \\
GS           & 0.4426400166562565   & 30.9448 & 0.87398 \\
Blending     & 0.12305350661515045  & 22.2765 & 0.46608 \\
\elastix     & 0.5668404588112618   & 32.951  & 0.89829 \\
Locally distorted  &
               0.028323699421965318 & 19.8731 & 0.39437 \\
Ground truth & 0.5169049621530698   & 31.4465 & 0.87478 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[tbh]
\centering
\caption{Numerical values for the evaluation of the registrations on the EM data set, in the middle of the series (Figs. \ref{fig:eval-em-1}, \ref{fig:eval-em-2}). In Jaccard measure, we global thresholds of~100 and 150, as indicated with \enquote{J~100} and \enquote{J~150}. \enquote{Locally distorted} means images resulting from our method applied to normalized ground truth for \emph{local} distortions, but no global rigid transformations were used in this case. The actual registrations operate on images that were also rigidly transformed. Notice the differences between the rigid-only and non-rigid methods. Notice also the differences between both rigid versions as well as the impact of normalization and 8~bit discretization on the ground truth values.\newline%
The larger the values, the better---up to the ground truth value.}
\label{tab:eval-em}
\begin{tabular}{r S[round-mode = figures, round-precision = 3, table-format = 1.3] S[round-mode = figures, round-precision = 3, table-format = 1.3] S[round-mode = figures, round-precision = 3, table-format = 2.1] S[round-mode = figures, round-precision = 3, table-format = 1.3]}
\multicolumn{5}{c}{\emph{EM}} \\
\toprule
%Method       & Jaccard & PSNR & SSIM \\
\multicolumn{1}{c}{Method}     & {J~100}      & {J~150}      & {PSNR}  & {SSIM} \\
\midrule
Rigid-SIFT   & 0.9276081431119362 & 0.9225060245713806 & 15.5516 & 0.81254 \\
Rigid-SURF   & 0.924928999536801  & 0.9254346345398599 & 16.4699 & 0.77089 \\
Deform-SURF  & 0.9745534130998824 & 0.9761642655434835 & 22.3554 & 0.88543 \\ 
GS           & 0.9644736716429315 & 0.9671098323246354 & 21.843  & 0.88490 \\
Blending     & 0.9250378431658511 & 0.9192509609315263 & 16.3058 & 0.81581 \\
\elastix     & 0.978667106853811  & 0.9814930078003433 & 23.4023 & 0.90006 \\
Locally distorted
             & 0.9098030739673391 & 0.9064435973320805 & 13.8757 & 0.77175 \\
Ground truth, norm'ed
             & 0.9739544464013851 & 0.9742027371979077 & 21.8014 & 0.92483 \\
         % 0.9776167641266931 for 499-500 @ 150
Ground truth, original
             & 0.9995468762972292 & 0.9816452794000238 & 37.0671 & 0.86913 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[tbh]
\centering
\caption{Numerical values for the evaluation of the registrations on the LS data set, in the middle of the series (Figs. \ref{fig:eval-ls-1}, \ref{fig:eval-ls-2}.). In Jaccard measure, we used a global threshold of~100. Low values in blending transforms and in rigid-only methods can be explained by residual shifts. Notice the improvements in non-rigid methods. The shorthand $s$ stands for \enquote{stretch}.\newline%
The larger the values, the better---up to the ground truth value.}
\label{tab:eval-ls}
\begin{tabular}{r S[round-mode = figures, round-precision = 3, table-format = 1.3] S[round-mode = figures, round-precision = 3, table-format = 2.1] S[round-mode = figures, round-precision = 3, table-format = 1.3]}
\multicolumn{4}{c}{\emph{LS}} \\
\toprule
%Method       & Jaccard & PSNR & SSIM \\
\multicolumn{1}{c}{Method}       & {Jaccard} & {PSNR}   & {SSIM}   \\
\midrule
Rigid-SIFT           & 0.9293306568382256    & 24.8826  & 0.75905  \\
Rigid-SURF           & 0.5994671672065636    & 19.0251  & 0.47885  \\
Deform-SURF, $s=\num{e-3}$
             & 0.9302626964887405    & 36.0127  & 0.96236  \\
Deform-SURF, $s=\num{5e-3}$
             & 0.9325623530318801    & 36.356   & 0.96456  \\
Deform-SURF, $s=\num{e-2}$
             & 0.9326951353526598    & 36.3505  & 0.96448  \\
GS                   & 0.9404650887398789    & 37.0971  & 0.97291  \\
Blending             & 0.9281149307337095    & 25.3271  & 0.77684  \\
\elastix             & 0.9409431110127936    & 37.1795  & 0.96830  \\
Locally distorted    & 0.909083130281718     & 23.3455  & 0.70967  \\
Ground truth, norm'ed& 0.9814964512292671    & 40.3112  & 0.94642  \\
\bottomrule
\end{tabular}
\end{table}

\begin{figure}[!t]
\centering
\setlength{\myfig}{0.2\linewidth-0.001\linewidth-2pt-0.2em}
\setlength{\tabcolsep}{1pt}
\begin{tabular}{m{1em} m{\myfig} m{\myfig} m{\myfig} m{\myfig} m{\myfig}}
& \multicolumn{1}{c}{Image} & \multicolumn{1}{c}{Dice} & \multicolumn{1}{c}{PSNR} & \multicolumn{1}{c}{SSIM} & \multicolumn{1}{c}{Flow} \\
\rot{\myfig}{Rigid-SIFT} &
\scalebarme{%
\includegraphics[height=\myfig]{image/CT/eval/ct_sift_old/crop_gray_rigid2_0_300.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_ct-500.png}} &
\includegraphics[height=\myfig]{image/CT/eval/ct_sift_old/crop_pair__ct-sift-rigid_300-301_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_sift_old/crop_psnr__ct-sift-rigid_300-301_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_sift_old/crop_ssim_full__ct-sift-rigid_300-301_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_sift_old/crop_flow_CROP__ct-sift-rigid_300-301_.png} 
\\

\rot{\myfig}{Rigid-SURF} &
\scalebarme{%
\includegraphics[height=\myfig]{image/CT/eval/ct_surf_rigid/crop_gray_rigid2_0_0300.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_ct-500.png}} &
\includegraphics[height=\myfig]{image/CT/eval/ct_surf_rigid/crop_pair__ct-surf-rigid_300-301_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_surf_rigid/crop_psnr__ct-surf-rigid_300-301_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_surf_rigid/crop_ssim_full__ct-surf-rigid_300-301_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_surf_rigid/crop_flow_CROP__ct-surf-rigid_300-301_.png}
\\

\rot{\myfig}{~~Deform-SURF} &
\scalebarme{%
\includegraphics[height=\myfig]{image/CT/eval/ct_surf_deform-std/crop_gray_warped2_3_0300.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_ct-500.png}} &
\includegraphics[height=\myfig]{image/CT/eval/ct_surf_deform-std/crop_pair__ct-surf-deform_300-301_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_surf_deform-std/crop_psnr__ct-surf-deform_300-301_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_surf_deform-std/crop_ssim_full__ct-surf-deform_300-301_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_surf_deform-std/crop_flow_CROP__ct-surf-deform_300-301_.png}
\\

\rot{\myfig}{GS} &
\scalebarme{%
\includegraphics[height=\myfig]{image/CT/eval/ct_sg/crop_gray_rigid2_0_0300_def.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_ct-500.png}} &
\includegraphics[height=\myfig]{image/CT/eval/ct_sg/crop_pair__ct-sg_300-301_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_sg/crop_psnr__ct-sg_300-301_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_sg/crop_ssim_full__ct-sg_300-301_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_sg/crop_flow_CROP__ct-sg_300-301_.png} 
\\

\rot{\myfig}{Ground truth} &
\scalebarme{%
\includegraphics[height=\myfig]{image/CT/eval/ct_orig/crop_gray_191146-1_E1-denoise_000650.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_ct-500.png}} &
\includegraphics[height=\myfig]{image/CT/eval/ct_orig/crop_pair__ct-orig_orig-index_650-651_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_orig/crop_psnr__ct-orig_orig-index_650-651_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_orig/crop_ssim_full__ct-orig_orig-index_650-651_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_orig/crop_flow_CROP__ct-orig_orig-index_650-651_.png}
\\

& \multicolumn{1}{c}{Image} & \multicolumn{1}{c}{Dice} & \multicolumn{1}{c}{PSNR} & \multicolumn{1}{c}{SSIM} & \multicolumn{1}{c}{Flow} \\
\end{tabular}

\caption{Evaluation of CT data set with image measures, part~1. Continued in Fig.~\ref{fig:eval-ct-2}. All scale bars are \SI{1}{\milli\meter}.}
\label{fig:eval-ct-1}
\setlength{\tabcolsep}{\tabcolbackup}
\end{figure}
\begin{figure}[!t]
\centering
%\newlength{\myfig}
\setlength{\myfig}{0.2\linewidth-0.001\linewidth-2pt-0.2em}
\setlength{\tabcolsep}{1pt}
\begin{tabular}{m{1em} m{\myfig} m{\myfig} m{\myfig} m{\myfig} m{\myfig}}
& \multicolumn{1}{c}{Image} & \multicolumn{1}{c}{Dice} & \multicolumn{1}{c}{PSNR} & \multicolumn{1}{c}{SSIM} & \multicolumn{1}{c}{Flow} \\

\rot{\myfig}{Blending} &
\scalebarme{%
\includegraphics[height=\myfig]{image/CT/eval/ct_funatomi/crop_gray_out0899.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_ct-500.png}} &
\includegraphics[height=\myfig]{image/CT/eval/ct_funatomi/crop_pair__ct-funatomi_899-900_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_funatomi/crop_psnr__ct-funatomi_899-900_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_funatomi/crop_ssim_full__ct-funatomi_899-900_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_funatomi/crop_flow_CROP__ct-funatomi_899-900_.png}
\\

\rot{\myfig}{\elastix} &
\scalebarme{%
\includegraphics[height=\myfig]{image/CT/eval/ct_el_prerigid_ol/crop_gray_el_0300.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_ct-500.png}} &
\includegraphics[height=\myfig]{image/CT/eval/ct_el_prerigid_ol/crop_pair__ct-el_OL_300-301_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_el_prerigid_ol/crop_psnr__ct-el_OL_300-301_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_el_prerigid_ol/crop_ssim_full__ct-el_OL_300-301_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_el_prerigid_ol/crop_flow_CROP__ct-el_OL_300-301_.png}
\\

\rot{\myfig}{Local only} &
\scalebarme{%
\includegraphics[height=\myfig]{image/CT/eval/ct_distort-only/crop_gray_191146-1_distort_only_000650.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_ct-500.png}} &
\includegraphics[height=\myfig]{image/CT/eval/ct_distort-only/crop_pair__ct-distort-only_orig-index_650-651_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_distort-only/crop_psnr__ct-distort-only_orig-index_650-651_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_distort-only/crop_ssim_full__ct-distort-only_orig-index_650-651_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_distort-only/crop_flow_CROP__ct-distort-only_orig-index_650-651_.png}
\\

\rot{\myfig}{Ground truth} &
\scalebarme{%
\includegraphics[height=\myfig]{image/CT/eval/ct_orig/crop_gray_191146-1_E1-denoise_000650.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_ct-500.png}} &
\includegraphics[height=\myfig]{image/CT/eval/ct_orig/crop_pair__ct-orig_orig-index_650-651_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_orig/crop_psnr__ct-orig_orig-index_650-651_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_orig/crop_ssim_full__ct-orig_orig-index_650-651_.png} &
\includegraphics[height=\myfig]{image/CT/eval/ct_orig/crop_flow_CROP__ct-orig_orig-index_650-651_.png}
\\

& \multicolumn{1}{c}{Image} & \multicolumn{1}{c}{Dice} & \multicolumn{1}{c}{PSNR} & \multicolumn{1}{c}{SSIM} & \multicolumn{1}{c}{Flow} \\
\end{tabular}

\caption{Evaluation of CT data set with image measures, part~2. Continued from Fig.~\ref{fig:eval-ct-1}. \enquote{Local only} means the distorted ground truth, but with no global transforms applied. The registrations' input had global transforms applied. All scale bars are \SI{1}{\milli\meter}.}
\label{fig:eval-ct-2}
\setlength{\tabcolsep}{\tabcolbackup}
\end{figure}


%%%%% EM
\begin{figure}[t]
\centering
\setlength{\myfig}{0.2\linewidth-0.001\linewidth-2pt-0.2em}
\setlength{\tabcolsep}{1pt}
\begin{tabular}{m{1em} m{\myfig} m{\myfig} m{\myfig} m{\myfig} m{\myfig}}
& \multicolumn{1}{c}{Image} & \multicolumn{1}{c}{Dice} & \multicolumn{1}{c}{PSNR} & \multicolumn{1}{c}{SSIM} & \multicolumn{1}{c}{Flow} \\


\rot{\myfig}{Rigid-SIFT} &
\scalebarme{%
\includegraphics[height=\myfig]{image/EM/eval/em_sift/crop_gray_rigid2_0_500.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_em-500.png}} &
\includegraphics[height=\myfig]{image/EM/eval/em_sift/crop_pair__em-sift-rigid_500-501_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_sift/crop_psnr__em-sift-rigid_500-501_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_sift/crop_ssim_full__em-sift-rigid_500-501_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_sift/crop_flow_CROP__em-sift-rigid_500-501_.png}
\\

\rot{\myfig}{Rigid-SURF} &
\scalebarme{%
\includegraphics[height=\myfig]{image/EM/eval/em_surf_rigid/crop_gray_rigid2_0_0500.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_em-500.png}} &
\includegraphics[height=\myfig]{image/EM/eval/em_surf_rigid/crop_pair__em-surf-rigid_500-501_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_surf_rigid/crop_psnr__em-surf-rigid_500-501_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_surf_rigid/crop_ssim_full__em-surf-rigid_500-501_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_surf_rigid/crop_flow_CROP__em-surf-rigid_500-501_.png}
\\

\rot{\myfig}{Deform-SURF} &
\scalebarme{%
\includegraphics[height=\myfig]{image/EM/eval/em_surf_dist-NORM/crop_gray_warped2_3_0500.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_em-500.png}} &
\includegraphics[height=\myfig]{image/EM/eval/em_surf_dist-NORM/crop_pair__em-surf-dist-norm_500-501_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_surf_dist-NORM/crop_psnr__em-surf-dist-norm_500-501_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_surf_dist-NORM/crop_ssim_full__em-surf-dist-norm_500-501_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_surf_dist-NORM/crop_flow_CROP__em-surf-dist-norm_500-501_.png}
\\


\rot{\myfig}{GS} &
\scalebarme{%
\includegraphics[height=\myfig]{image/EM/eval/em_sg/crop_gray_rigid2_0_0500_def.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_em-500.png}} &
\includegraphics[height=\myfig]{image/EM/eval/em_sg/crop_pair__em-sg_500-501_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_sg/crop_psnr__em-sg_500-501_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_sg/crop_ssim_full__em-sg_500-501_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_sg/crop_flow_CROP__em-sg_500-501_.png}
\\


\rot{\myfig}{Blending} &
\scalebarme{%
\includegraphics[height=\myfig]{image/EM/eval/em_funatomi/crop_gray_out1499.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_em-500.png}} &
\includegraphics[height=\myfig]{image/EM/eval/em_funatomi/crop_pair__em-funatomi_1499-1500__500-501_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_funatomi/crop_psnr__em-funatomi_1499-1500__500-501_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_funatomi/crop_ssim_full__em-funatomi_1499-1500__500-501_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_funatomi/crop_flow_CROP__em-funatomi_1499-1500__500-501_.png}
\\


\rot{\myfig}{Gr.~truth, norm.} &
\scalebarme{%
\includegraphics[height=\myfig]{image/EM/eval/em_orig-norm/crop_gray_norm_0500-dump.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_em-500.png}} &
\includegraphics[height=\myfig]{image/EM/eval/em_orig-norm/crop_pair__em-orig-norm_499-500_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_orig-norm/crop_psnr__em-orig-norm_499-500_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_orig-norm/crop_ssim_full__em-orig-norm_499-500_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_orig-norm/crop_flow_CROP__em-orig-norm_499-500_.png}
\\


& \multicolumn{1}{c}{Image} & \multicolumn{1}{c}{Dice} & \multicolumn{1}{c}{PSNR} & \multicolumn{1}{c}{SSIM} & \multicolumn{1}{c}{Flow} \\

\end{tabular}

\caption{Evaluation of EM data set with image measures, part~1. Continued in Fig.~\ref{fig:eval-em-2}. All scale bars are \SI{10}{\micro\meter}.}
\label{fig:eval-em-1}
\setlength{\tabcolsep}{\tabcolbackup}
\end{figure}
\begin{figure}[tb]
\centering
\setlength{\myfig}{0.2\linewidth-0.001\linewidth-2pt-0.2em}
\setlength{\tabcolsep}{1pt}
\begin{tabular}{m{1em} m{\myfig} m{\myfig} m{\myfig} m{\myfig} m{\myfig}}
& \multicolumn{1}{c}{Image} & \multicolumn{1}{c}{Dice} & \multicolumn{1}{c}{PSNR} & \multicolumn{1}{c}{SSIM} & \multicolumn{1}{c}{Flow} \\


\rot{\myfig}{\elastix} &
\scalebarme{%
\includegraphics[height=\myfig]{image/EM/eval/em_el_prerigid_ol/crop_gray_el_0500.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_em-500.png}} &
\includegraphics[height=\myfig]{image/EM/eval/em_el_prerigid_ol/crop_pair__em-el_500-501_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_el_prerigid_ol/crop_psnr__em-el_500-501_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_el_prerigid_ol/crop_ssim_full__em-el_500-501_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_el_prerigid_ol/crop_flow_CROP__em-el_500-501_.png}
\\

\rot{\myfig}{Local only} &
\scalebarme{%
\includegraphics[height=\myfig]{image/EM/eval/em_distort-only/crop_gray_local_0500.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_em-500.png}} &
\includegraphics[height=\myfig]{image/EM/eval/em_distort-only/crop_pair__em-LOCAL_ONLY_500-501_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_distort-only/crop_psnr__em-LOCAL_ONLY_500-501_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_distort-only/crop_ssim_full__em-LOCAL_ONLY_500-501_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_distort-only/crop_flow_CROP__em-LOCAL_ONLY_500-501_.png}
\\

\rot{\myfig}{Gr.~truth, norm.} &
\scalebarme{%
\includegraphics[height=\myfig]{image/EM/eval/em_orig-norm/crop_gray_norm_0500-dump.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_em-500.png}} &
\includegraphics[height=\myfig]{image/EM/eval/em_orig-norm/crop_pair__em-orig-norm_499-500_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_orig-norm/crop_psnr__em-orig-norm_499-500_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_orig-norm/crop_ssim_full__em-orig-norm_499-500_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_orig-norm/crop_flow_CROP__em-orig-norm_499-500_.png}
\\

\rot{\myfig}{Gr.~truth, orig.} &
\scalebarme{%
\includegraphics[height=\myfig]{image/EM/eval/em_orig-16bit/crop_gray_17-837b_bi3_rs+1+150_smROI_ROI01_adg_0500.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_em-500.png}} &
\includegraphics[height=\myfig]{image/EM/eval/em_orig-16bit/crop_pair__em-FULL-ORIG-16bit__500-501_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_orig-16bit/crop_psnr__em-FULL-ORIG-16bit__500-501_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_orig-16bit/crop_ssim_full__em-FULL-ORIG-16bit__500-501_.png} &
\includegraphics[height=\myfig]{image/EM/eval/em_orig-16bit/crop_flow_CROP__em-FULL-ORIG-16bit__500-501_.png}
\\


& \multicolumn{1}{c}{Image} & \multicolumn{1}{c}{Dice} & \multicolumn{1}{c}{PSNR} & \multicolumn{1}{c}{SSIM} & \multicolumn{1}{c}{Flow} \\

\end{tabular}
\caption{Evaluation of EM data set with image measures, part~2. Continued from Fig.~\ref{fig:eval-em-1}. All scale bars are \SI{10}{\micro\meter}.}
\label{fig:eval-em-2}
\setlength{\tabcolsep}{\tabcolbackup}
\end{figure}

%%%%% LS
\begin{figure}[!t]
\centering
\setlength{\myfig}{0.2\linewidth-0.001\linewidth-2pt-0.2em}
\setlength{\tabcolsep}{1pt}
\begin{tabular}{m{1em} m{\myfig} m{\myfig} m{\myfig} m{\myfig} m{\myfig}}
& \multicolumn{1}{c}{Image} & \multicolumn{1}{c}{Dice} & \multicolumn{1}{c}{PSNR} & \multicolumn{1}{c}{SSIM} & \multicolumn{1}{c}{Flow} \\


\rot{\myfig}{Rigid-SIFT} &
\scalebarme{%
\includegraphics[height=\myfig]{image/LS/eval/ls_sift-rigid/crop_gray_rigid2_0_150.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_ls-500.png}} &
\includegraphics[height=\myfig]{image/LS/eval/ls_sift-rigid/crop_pair__ls-sift-rigid_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_sift-rigid/crop_psnr__ls-sift-rigid_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_sift-rigid/crop_ssim_full__ls-sift-rigid_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_sift-rigid/crop_flow_CROP__ls-sift-rigid_150-151_.png}
\\

\rot{\myfig}{GS} &
\scalebarme{%
\includegraphics[height=\myfig]{image/LS/eval/ls_sg/crop_gray_rigid2_0_0150_def.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_ls-500.png}} &
\includegraphics[height=\myfig]{image/LS/eval/ls_sg/crop_pair__ls-sg_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_sg/crop_psnr__ls-sg_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_sg/crop_ssim_full__ls-sg_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_sg/crop_flow_CROP__ls-sg_150-151_.png}
\\

\rot{\myfig}{Blending} &
\scalebarme{%
\includegraphics[height=\myfig]{image/LS/eval/ls_funatomi/crop_gray_out0449.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_ls-500.png}} &
\includegraphics[height=\myfig]{image/LS/eval/ls_funatomi/crop_pair__ls-funatomi_449-450__150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_funatomi/crop_psnr__ls-funatomi_449-450__150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_funatomi/crop_ssim_full__ls-funatomi_449-450__150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_funatomi/crop_flow_CROP__ls-funatomi_449-450__150-151_.png}
\\

\rot{\myfig}{\elastix} &
\scalebarme{%
\includegraphics[height=\myfig]{image/LS/eval/ls_el_prerigid_ol/crop_gray_el_0150.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_ls-500.png}} &
\includegraphics[height=\myfig]{image/LS/eval/ls_el_prerigid_ol/crop_pair__ls-el_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_el_prerigid_ol/crop_psnr__ls-el_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_el_prerigid_ol/crop_ssim_full__ls-el_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_el_prerigid_ol/crop_flow_CROP__ls-el_150-151_.png}
\\


\rot{\myfig}{Local dist.} &
\scalebarme{%
\includegraphics[height=\myfig]{image/LS/eval/ls_local-only/crop_gray_local_0150.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_ls-500.png}} &
\includegraphics[height=\myfig]{image/LS/eval/ls_local-only/crop_pair__ls-local-only_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_local-only/crop_psnr__ls-local-only_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_local-only/crop_ssim_full__ls-local-only_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_local-only/crop_flow_CROP__ls-local-only_150-151_.png}
\\

\rot{\myfig}{Gr.~truth, norm.} &
\scalebarme{%
\includegraphics[height=\myfig]{image/LS/eval/ls_norm/crop_gray_norm_0150.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_ls-500.png}} &
\includegraphics[height=\myfig]{image/LS/eval/ls_norm/crop_pair__ls-ground-norm_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_norm/crop_psnr__ls-ground-norm_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_norm/crop_ssim_full__ls-ground-norm_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_norm/crop_flow_CROP__ls-ground-norm_150-151_.png}
\\

& \multicolumn{1}{c}{Image} & \multicolumn{1}{c}{Dice} & \multicolumn{1}{c}{PSNR} & \multicolumn{1}{c}{SSIM} & \multicolumn{1}{c}{Flow} \\


\end{tabular}
\caption{Evaluation of LS data set with image measures, part~1. The ground truth is normalized. Continued in Fig.~\ref{fig:eval-ls-2}. All scale bars are \SI{500}{\micro\meter}.}
\label{fig:eval-ls-1}
\setlength{\tabcolsep}{\tabcolbackup}
\end{figure}
\begin{figure}[!t]
\centering
\setlength{\myfig}{0.2\linewidth-0.001\linewidth-2pt-0.2em}
\setlength{\tabcolsep}{1pt}
\begin{tabular}{m{1em} m{\myfig} m{\myfig} m{\myfig} m{\myfig} m{\myfig}}
& \multicolumn{1}{c}{Image} & \multicolumn{1}{c}{Dice} & \multicolumn{1}{c}{PSNR} & \multicolumn{1}{c}{SSIM} & \multicolumn{1}{c}{Flow} \\

\rot{\myfig}{Rigid-SURF} &
\scalebarme{%
\includegraphics[height=\myfig]{image/LS/eval/ls_surf-rigid/crop_gray_rigid2_0_0150.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_ls-500.png}} &
\includegraphics[height=\myfig]{image/LS/eval/ls_surf-rigid/crop_pair__ls-surf-rigid_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_surf-rigid/crop_psnr__ls-surf-rigid_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_surf-rigid/crop_ssim_full__ls-surf-rigid_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_surf-rigid/crop_flow_CROP__ls-surf-rigid_150-151_.png}
\\


\rot{\myfig}{D.-SURF, std.} &
\scalebarme{%
\includegraphics[height=\myfig]{image/LS/eval/ls_surf-deform_std/crop_gray_warped2_3_0150.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_ls-500.png}} &
\includegraphics[height=\myfig]{image/LS/eval/ls_surf-deform_std/crop_pair__ls-surf-deform-std_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_surf-deform_std/crop_psnr__ls-surf-deform-std_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_surf-deform_std/crop_ssim_full__ls-surf-deform-std_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_surf-deform_std/crop_flow_CROP__ls-surf-deform-std_150-151_.png}
\\

\rot{\myfig}{D.-SURF, \num{e-3}} &
\scalebarme{%
\includegraphics[height=\myfig]{image/LS/eval/ls_surf-deform_1e-3/crop_gray_warped2_3_0150.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_ls-500.png}} &
\includegraphics[height=\myfig]{image/LS/eval/ls_surf-deform_1e-3/crop_pair__ls-surf-deform-1e-3_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_surf-deform_1e-3/crop_psnr__ls-surf-deform-1e-3_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_surf-deform_1e-3/crop_ssim_full__ls-surf-deform-1e-3_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_surf-deform_1e-3/crop_flow_CROP__ls-surf-deform-1e-3_150-151_.png}
\\

\rot{\myfig}{D.-SURF, \num{e-2}} &
\scalebarme{%
\includegraphics[height=\myfig]{image/LS/eval/ls_surf-deform_1e-2/crop_gray_warped2_3_0150.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_ls-500.png}} &
\includegraphics[height=\myfig]{image/LS/eval/ls_surf-deform_1e-2/crop_pair__ls-surf-deform-1e-2_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_surf-deform_1e-2/crop_psnr__ls-surf-deform-1e-2_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_surf-deform_1e-2/crop_ssim_full__ls-surf-deform-1e-2_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_surf-deform_1e-2/crop_flow_CROP__ls-surf-deform-1e-2_150-151_.png}
\\


\rot{\myfig}{Gr.~truth, norm.} &
\scalebarme{%
\includegraphics[height=\myfig]{image/LS/eval/ls_norm/crop_gray_norm_0150.png}}{%
\includegraphics[width=\myfig]{image/scalebars/scale_ls-500.png}} &
\includegraphics[height=\myfig]{image/LS/eval/ls_norm/crop_pair__ls-ground-norm_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_norm/crop_psnr__ls-ground-norm_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_norm/crop_ssim_full__ls-ground-norm_150-151_.png} &
\includegraphics[height=\myfig]{image/LS/eval/ls_norm/crop_flow_CROP__ls-ground-norm_150-151_.png}
\\

& \multicolumn{1}{c}{Image} & \multicolumn{1}{c}{Dice} & \multicolumn{1}{c}{PSNR} & \multicolumn{1}{c}{SSIM} & \multicolumn{1}{c}{Flow} \\

\end{tabular}
\caption{Evaluation of LS data set with image measures, part~2, mostly variations over \enquote{Deform-SURF}, abbreviated here as \enquote{D.-SURF}. We differentiate the \enquote{stretch} parameter of the non-rigid phase. The default value is the factor \num{5e-3} of the image size. We also test \enquote{Deform-SURF} with the values \num{e-3} and \num{e-2}. The ground truth is normalized. Continued from Fig.~\ref{fig:eval-ls-1}. All scale bars are \SI{500}{\micro\meter}.}
\label{fig:eval-ls-2}
\setlength{\tabcolsep}{\tabcolbackup}
\end{figure}

\label{sec:eval-pairs} We use two consecutive not distorted images from
the middle of the each series as a ground truth for the evaluation of
multiple registration methods. We also use two consecutive images at the
same positioning from the registrations' results. The input of the
registrations is the series in its completeness after the application of
distortions presented in this paper. Both local distortions and rigid
transformations were applied. Two consecutive result images from the
middle of the registered series are subject of the quality measures
Jaccard, PSNR and SSIM as outlined in section~\ref{sec:eval}. We also
utilize two consecutive locally distorted images to produce comparison
values. In the image-based evaluation we show a \xroi{500}{500} crop
from the image center to highlight details.

The tables below show the Jaccard, PSNR and SSIM values for the ground
truth (undistorted images), as well as the locally deformed images. In
part, the values for the normalized ground truth images were also given,
to give an idea about the impact of intensity variations on the ground
truth measures. Same intensity variations as in \enquote{normalized
ground truths} were also present in registrations' inputs.

Hence, the effect of the non-rigid registrations can be read as an
improvement between \enquote{locally distorted} and \enquote{normalized
ground truths,} but there was also a global rigid transformation.
Undoing it with a rigid registration might have lead to a worse starting
point for the non-rigid registration than \enquote{locally distorted.}

\hypertarget{results}{%
\subsubsection{Results}\label{results}}

\sisetup{round-mode = figures, round-precision = 3}

Basically, Figs.~\ref{fig:eval-ct-1} and~\ref{fig:eval-ct-2} show the
pair-wise image-based evaluations for the CT data set;
Figs.~\ref{fig:eval-em-1} and~\ref{fig:eval-em-2} show the pair-wise
evaluation for the EM data set; Figs.~\ref{fig:eval-ls-1}
and~\ref{fig:eval-ls-2} show the pair-wise evaluation for the LS data
set. Table~\ref{tab:eval-ct} shows the numerical values of the pair-wise
image-based metrics for CT; Table~\ref{tab:eval-em} shows these for EM;
Table~\ref{tab:eval-ls} for LS. The full-series evaluation follows in
section~\ref{full-series-evaluation}.

\hypertarget{ct-data-set}{%
\paragraph{CT data set}\label{ct-data-set}}

Consider Fig.~\ref{fig:eval-ct-1}. Both rigid-only methods leave some
incongruences, these are then greatly reduced by \enquote{Deform-SURF.}
\enquote{GS} also works on rigidly pre-registered input, but produces a
very different image of residual movements in optical flow
visualization. It reaches also very good values \wrt other measures,
\eg SSIM. The \elastix-based registration (Fig.~\ref{fig:eval-ct-2})
reaches even better values \wrt SSIM and PSNR. We see some more movement
in Dice visualization, but it is not reflected in Jaccard measure
(Tab.~\ref{tab:eval-ct}). The apparent reason might be the varying
thresholding methods. \enquote{Blending} has some residual movement, as
seen in PSNR and optical flow visualization. The goal of
\enquote{Blending} was a coarse alignment, hence the lower quality
measures. Notice, however, that it copes with the random global
transformations on its own, without the initial \enquote{Rigid-SURF}
stage. In \enquote{local only} we see some global movement with is a
residue of a local distortion at a larger scale. Not surprisingly, there
are still some residues of it left in rigid methods, as discussed above.

Consider the ground truth as the \enquote{ideal} image pair. Little
signal in PSNR means little change. It is also visible in the
visualizations as less red. SSIM and optical flow visualizations show
that these differences are local and evenly distributed across the
region. In registered images there are typically more differences; those
are also more concentrated in a region. Such concentrated
\enquote{change} means stronger local transformations.

The visualized differences in the ground truth appear to be less than in
most of the registration results (all in Fig.~\ref{fig:eval-ct-1}) and
also more scattered across the image: compare, \eg the optical flow
visualization between ground truth, \enquote{GS,} and
\enquote{Deform-SURF.} As for \elastix, there are \emph{less}
differences between two consecutive images than in the ground truth. The
SSIM and optical flow visualization of \elastix results show the
differing parts to be more concentrated in the certain areas (\eg the
bottom part and the first third part of the crop) when compared to the
same areas of the ground truth. Such a behavior is hinting at
overfitting. In the ground truth the \enquote{change} is more evenly
distributed across the image. (We can easily make statements about the
localization of the movement or local differences with the visualization
of optical flow. Optical flow highlights the movement across consecutive
images. However, in its present form, it is rather hard to make
statements about the \emph{magnitude} of the movement across multiple
visualizations. In this work we need to rely on other measures for a
comparable assessment.)
\dhcomment{I had a hard time understanding what is explained here. I think I still don't truly understand it, but this might just be because I have *no* experience with registration and registration measures.}

If we look at the numerical values, we observe that all three measures
are \emph{lower} for the ground truth than for \elastix. The verdict
appears to be that \elastix (with our parameter file) over-registers the
CT data set. However, there is still some noise in the data that is
irrelevant for real-world tasks. The noise, however, still contributes
to the measures and is also the subject of registration---we did not use
a mask. Such \enquote{unnecessary} alignments might explain the too
large values for \elastix. Still, the GS method is remarkable in how
close it gets to the values of the ground truth quality measures.

\hypertarget{em-data-set}{%
\paragraph{EM data set}\label{em-data-set}}

The differences between rigidly registered images with SIFT and SURF in
Fig.~\ref{fig:eval-em-1} appear to be the effect of different
normalizations---we were attempting to undo the individual normalization
of the image in inputs of the \enquote{Rigid-SURF} method. Again, we see
residual incongruences with rigid-only methods. Both
\enquote{Deform-SURF} (Fig.~\ref{fig:eval-em-1}) and
\elastix (Fig.~\ref{fig:eval-em-2}) have multiple small
\enquote{movements} in optical flow visualization, as opposed to a more
or less uniform color of a global shift. \enquote{Blending}
(Fig.~\ref{fig:eval-em-1}) shows somewhat uncompensated distortion in
the middle of the image, in Dice, SSIM, and optical flow visualizations.
It appears that in this method the effect of our local distortion
(Fig.~\ref{fig:eval-em-2}) has not been corrected completely, but the
random global transformation was undone well.

From the visualizations, \enquote{GS} (Fig.~\ref{fig:eval-em-1}) and
normalized ground truth have definitely less movement than,
\eg \enquote{Deform-SURF.} The movement in \enquote{GS} seems more
evenly distributed, normalized ground truth has a \enquote{hot spot} in
the optical flow visualization. Curiously, the original ground truth has
both more details (because it is not clamped-down 16~bit data) and more
movement can be detected therein (compare flows and SSIM of the
normalized and original ground truths). At the same time, PSNR is higher
with the original image pair.

Numerically, \elastix has best Jaccard measures (both at 100 and 150
thresholds, indicated with postfix in the following), PSNR, and SSIM
among all registrations. Especially with Jaccard~100,
\enquote{Deform-SURF} is a very close follow-up, at \SI{99.6}{\percent}
of the performance of \elastix. Now, if we look at the measures' values
of the objective ground truths---the luxury we did not have before in an
evaluation of registrations of serial sections---an issue is apparent.
Both Jaccard~100 and Jaccard~150 values for \elastix and (less so) for
\enquote{Deform-SURF} are \emph{higher} than for the normalized ground
truth! This issue might indicate an over-optimization by those
registrations.

To give some values, Jaccard~150 measure for \elastix is
\SI{0.74833198}{\percent} \emph{higher} than normalized ground truth,
same method has also \SI{7.3431064}{\percent} \emph{higher} PSNR than
normalized ground truth; \enquote{Deform-SURF} reaches
\SI{95.739758}{\percent} of the normalized ground truth SSIM. Notably,
from the visualizations we would deem \enquote{GS} as a very good
registration, comparable, if not beating \elastix. But numerically,
\elastix has much higher values.

\hypertarget{ls-data-set}{%
\paragraph{LS data set}\label{ls-data-set}}

In Figure~\ref{fig:eval-ls-1} we see a larger movement in the rigid
method. It originates from our local distortions in the region of
interest (\enquote{Local dist.}), but cannot be undone with rigid
methods only. \enquote{Blending} still suffers from these distortions,
but restores the coarse correspondence well. \enquote{GS} recovers very
well from those local movements, however it might over-register, based
on visual comparison with normalized ground truth. Both in optical flow
visualizations for \enquote{GS} and for the ground truth we see multiple
small \enquote{movements,} originating from the fact that we compare two
consecutive non-equal images. However, \enquote{GS} shows \emph{less}
movement than ground truth, hence our suspicion. Numerical values would
provide more clarity, we will look at them next. As for \elastix, Dice,
PSNR, and SSIM visualizations look very good, similar as in
\enquote{GS.} In \elastix, the visualization of optical flow appears in
general to be lower than the ground truth, but it also shows a
\enquote{hot spot} at the top part of the image. However, as already
mentioned, we should be careful with such comparisons between optical
flow visualizations.

Figure~\ref{fig:eval-ls-2} shows quite confident results from
\enquote{Deform-SURF,} but the \enquote{Rigid-SURF} is even worse than
\enquote{Rigid-SIFT} (Fig.~\ref{fig:eval-ls-1}). We use three different
values for the non-linear \enquote{stretch} in the non-rigid
feature-based registration method \enquote{Deform-SURF.} The
\enquote{stretch} values we state are a factor of image size in pixels,
limiting the magnitude of the \enquote{movement} in the non-linear
registration. When the deformation magnitude is apparently too small
(\num{e-3}), SSIM (and less so, PSNR) visualizations are slightly worse,
but the optical flow shows the problem \enquote{hot spot} near the
center of the image. The \enquote{standard} magnitude of \num{5e-3} is
already much better and does not have the aforementioned problem. An
even larger magnitude \num{e-2} also looks similar to the standard
setting. Whether those two parameters in \enquote{Deform-SURF}
over-register can be determined from the numerical values below. For
now, we can say that normalized ground truth is slightly better in PSNR,
Dice, and SSIM, but appears more \enquote{noisy,} but also more
\enquote{even} than \enquote{Deform-SURF.} We deem the variations in
intensity of the registered images in different methods as originating
from a rather needed normalization before registration.

Table~\ref{tab:eval-ls} shows numerical values. The Jaccard measure is
computed with threshold~100. \enquote{Rigid-SIFT} was very successful
\wrt Jaccard measure, but PSNR and SSIM are lower than in a typical
non-rigid registration. In a contrast, \enquote{Rigid-SURF} is quite bad
\wrt all three measures. Still, it manages to be a good input for the
non-rigid methods \enquote{Deform-SURF,} GS, and \elastix. Comparing
different \enquote{stretch} values with \enquote{Deform-SURF}
numerically, we see that the default value of \num{5e-3} is slightly
better than the larger value. Too small \enquote{stretch} decreases the
measures slightly, but it is still better than all rigid methods, for
PSNR and SSIM with a larger margin. The \enquote{Blending} method has
some problems, also evident in visualizations. We discussed this issue
above.

The methods \enquote{GS} and \elastix are very similar \wrt Jaccard
measure. Interestingly, PSNR is slightly higher with \elastix, but SSIM
is higher with \enquote{GS.} Both \enquote{GS} and \elastix have better
numerical values than all \enquote{Deform-SURF} methods tested
here---but what about the ground truth?

When compared to the (normalized) ground truth, Jaccard and PSNR
measures in all registrations are lower. Still, the Jaccard measures for
\enquote{GS} and \elastix are closer to the ground truth than in other
methods. However, the SSIM value for \enquote{Deform-SURF} is less than
\SI{2}{\percent} \emph{larger} than the actual SSIM for the normalized
ground truth image pair. Still, \enquote{GS} and \elastix have
\emph{even larger} SSIM values than the ground truth:
\SI{2.3118700}{\percent} and \SI{2.7989687}{\percent} correspondingly.
Such larger SSIM values might signal over-registration.

\hypertarget{special-cases}{%
\subsubsection{Special cases}\label{special-cases}}

For the above evaluation we intentionally picked the center of a series
and a clearly defined region. Now we would like to separately highlight
some especially good of bad consecutive image pairs in
Fig.~\ref{fig:special}. This is a subjective selection of image pairs,
as contrasted with the previous section.

In panel~\subref{fig:special-a} a~larger global shift in non-linear
distortion phase of the registrations' input is shown. It is CT data
set, sections 95--96, Dice visualization. Fig.~\subref{fig:special-b}
shows uncorrected global movement in \elastix-based registration, same
data set, sections 99--100, Dice visualization. There is
a~\enquote{floppy end} in \elastix result \subref{fig:special-c}, from
same data set, sections 305--306, Dice visualization. Mostly the
registration is good, but in the depicted region the offsets are much
larger.

In panels~\subref{fig:special-surf-good-1},
\subref{fig:special-surf-good-2} the measures of an~interesting image
pair from \enquote{Deform-SURF} are depicted. We show Dice
\subref{fig:special-surf-good-1} and optical flow
\subref{fig:special-surf-good-2} visualizations from the same region.
There \emph{is} some movement, but is it all explainable with the
\enquote{natural} differences in consecutive images?

The areas with little tissue (as found in our EM series near its end)
are a greater challenge for the feature-based methods, as
Figs.~\subref{fig:special-em-fail1}, \subref{fig:special-em-fail2} show.
We see there a failure of the feature-based SIFT method to find a
correct rigid alignment. Full images from EM data set, sections
702--703, are shown. The probable reason is the low number of viable key
points.

Subfigures~\subref{fig:special-sg-good-1}--\subref{fig:special-sg-good-3}
show a small evaluation of a particularly good GS-registered image pair,
LS data set, images 161--162. We show there Dice visualization, PSNR,
and SSIM, respectively, for the same region. Notice the low values and
very few differences.

\begin{figure}[tb]
%% CT 1000
\subfloat[][CT, local dist.]{\label{fig:special-a}%
\scalebarme{%
\includegraphics[width=0.199\linewidth]{image/CT/specials/input/special-crop_pair.png}}{%
\includegraphics[width=0.199\linewidth]{image/scalebars/scale_ct-13a.png}}}\hfill%
%% CT 500
\subfloat[][CT, \elastix]{\label{fig:special-b}%
\scalebarme{%
\includegraphics[width=0.199\linewidth]{image/CT/specials/elastix/crop_pair__ct-special_el_099-100.png}}{%
\includegraphics[width=0.199\linewidth]{image/scalebars/scale_ct-500.png}}}\hfill%
%% CT 1000
\subfloat[][CT, \elastix]{\label{fig:special-c}%
\scalebarme{\includegraphics[width=0.199\linewidth]{image/CT/specials/elastix/special-crop_el_pair_305-306.png}}{%
\includegraphics[width=0.199\linewidth]{image/scalebars/scale_ct-13a.png}}}\hfill%
%% CT 500
\subfloat[][CT, \enquote{Deform-SURF}]{\label{fig:special-surf-good-1}%
\scalebarme{\includegraphics[width=0.199\linewidth]{image/CT/specials/surf-deform/crop_pair__ct-special_surf-deform_348-349.png}}{%
\includegraphics[width=0.199\linewidth]{image/scalebars/scale_ct-500.png}}}\hfill%
%% CT 500
\subfloat[][CT, \enquote{Deform-SURF}]{\label{fig:special-surf-good-2}%
\scalebarme{\includegraphics[width=0.199\linewidth]{image/CT/specials/surf-deform/crop_flow_CROP__ct-special_surf-deform_348-349.png}}{%
\includegraphics[width=0.199\linewidth]{image/scalebars/scale_ct-500.png}}}

%% EM 1500
\subfloat[][EM, \enquote{Rigid-SIFT}]{\label{fig:special-em-fail1}%
\scalebarme{%
\includegraphics[width=0.199\linewidth]{image/EM/specials/rigid-sift/fail_rigid_702.png}}{%
\includegraphics[width=0.199\linewidth]{image/scalebars/scale_em-13f.png}}}\hfill%
%% EM 1500
\subfloat[][EM, \enquote{Rigid-SIFT}]{\label{fig:special-em-fail2}%
\scalebarme{%
\includegraphics[width=0.199\linewidth]{image/EM/specials/rigid-sift/fail_rigid_703.png}}{%
\includegraphics[width=0.199\linewidth]{image/scalebars/scale_em-13f.png}}}\hfill%
%% all LS 500
\subfloat[][LS, \enquote{GS}]{\label{fig:special-sg-good-1}%
\scalebarme{%
\includegraphics[width=0.199\linewidth]{image/LS/specials/sg/crop_pair__ls-special_sg_161-162.png}}{%
\includegraphics[width=0.199\linewidth]{image/scalebars/scale_ls-500.png}}}\hfill%
\subfloat[][LS, \enquote{GS}]{\label{fig:special-sg-good-2}%
\scalebarme{%
\includegraphics[width=0.199\linewidth]{image/LS/specials/sg/crop_psnr__ls-special_sg_161-162.png}}{%
\includegraphics[width=0.199\linewidth]{image/scalebars/scale_ls-500.png}}}\hfill%
\subfloat[][LS, \enquote{GS}]{\label{fig:special-sg-good-3}%
\scalebarme{%
\includegraphics[width=0.199\linewidth]{image/LS/specials/sg/crop_ssim_full__ls-special_sg_161-162.png}}{%
\includegraphics[width=0.199\linewidth]{image/scalebars/scale_ls-500.png}}}
\caption{Special cases, especially good or bad image pairs.\newline%
Scale bars are: \protect\subref{fig:special-a}$=$\SI{1}{\milli\meter},
\protect\subref{fig:special-b}$=$\SI{500}{\micro\meter},
\protect\subref{fig:special-c}$=$\SI{1}{\milli\meter},
\protect\subref{fig:special-surf-good-1}$=$\SI{500}{\micro\meter},
\protect\subref{fig:special-surf-good-2}$=$\SI{500}{\micro\meter},
\protect\subref{fig:special-em-fail1}$=$\SI{50}{\milli\meter},
\protect\subref{fig:special-em-fail2}$=$\SI{50}{\milli\meter},
\protect\subref{fig:special-sg-good-1}--\protect\subref{fig:special-sg-good-3}$=$\SI{500}{\micro\meter}.}
\label{fig:special}
\end{figure}


==> image/CT/eval/Funatomi_20201028/Makefile <==
SHELL = bash
.ONESHELL:

left=out0899.png
right=out0900.png
file_suffix=_ct-funatomi-NEW_899-900_

left_png=$(left:.tif=.png)
right_png=$(right:.tif=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL : psnr_FULL_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../../../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../../../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../../../code/$@ .

jaccard.py :
	-ln -s ../../../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/CT/eval/Funatomi_20201028/Makefile_ <==
SHELL = bash
.ONESHELL:

left=out0899.png
right=out0900.png
file_suffix=_ct-funatomi_899-900_

left_png=$(left:.tif=.png)
right_png=$(right:.tif=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/CT/eval/ct_benchmark-input/Makefile <==
SHELL = bash
.ONESHELL:

left=input_0300.png
right=input_0301.png
file_suffix=_ct-input_300-301_

left_png=$(left:.tif=.png)
right_png=$(right:.tif=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 150 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/CT/eval/ct_distort-only/Makefile <==
SHELL = bash
.ONESHELL:

left=191146-1_distort_only_000650.png
right=191146-1_distort_only_000651.png
file_suffix=_ct-distort-only_orig-index_650-651_

left_png=$(left:.tif=.png)
right_png=$(right:.tif=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/CT/eval/ct_el_prerigid_ol/Makefile <==
SHELL = bash
.ONESHELL:

left=el_0300.png
right=el_0301.png
file_suffix=_ct-el_OL_300-301_

left_png=$(left:.tif=.png)
right_png=$(right:.tif=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/CT/eval/ct_funatomi/Makefile <==
SHELL = bash
.ONESHELL:

left=out0899.png
right=out0900.png
file_suffix=_ct-funatomi_899-900_

left_png=$(left:.tif=.png)
right_png=$(right:.tif=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/CT/eval/ct_orig/Makefile <==
SHELL = bash
.ONESHELL:

left=191146-1_E1-denoise_000650.png
right=191146-1_E1-denoise_000651.png
file_suffix=_ct-orig_orig-index_650-651_

left_png=$(left:.tif=.png)
right_png=$(right:.tif=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/CT/eval/ct_sg/Makefile <==
SHELL = bash
.ONESHELL:

left=rigid2_0_0300_def.tif
right=rigid2_0_0301_def.tif
file_suffix=_ct-sg_300-301_

left_png=$(left:.tif=.png)
right_png=$(right:.tif=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/CT/eval/ct_sift_old/Makefile <==
SHELL = bash
.ONESHELL:

left=rigid2_0_300.tiff
right=rigid2_0_301.tiff
file_suffix=_ct-sift-rigid_300-301_

left_png=$(left:.tiff=.png)
right_png=$(right:.tiff=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/CT/eval/ct_surf_deform-std/Makefile <==
SHELL = bash
.ONESHELL:

left=warped2_3_0300.tiff
right=warped2_3_0301.tiff
file_suffix=_ct-surf-deform_300-301_

left_png=$(left:.tiff=.png)
right_png=$(right:.tiff=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/CT/eval/ct_surf_rigid/Makefile <==
SHELL = bash
.ONESHELL:

left=rigid2_0_0300.tiff
right=rigid2_0_0301.tiff
file_suffix=_ct-surf-rigid_300-301_

left_png=$(left:.tiff=.png)
right_png=$(right:.tiff=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/CT/specials/elastix/Makefile <==
SHELL = bash
.ONESHELL:

left=el_0099.png
right=el_0100.png
file_suffix=_ct-special_el_099-100

left_png=$(left:.tif=.png)
right_png=$(right:.tif=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../../../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../../../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../../../code/$@ .

jaccard.py :
	-ln -s ../../../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/CT/specials/elastix/Makefile_ <==
SHELL = bash
.ONESHELL:

left=191146-1_distort_only_000445.png
right=191146-1_distort_only_000446.png
file_suffix=_ct-special_orig-num_445-446_

left_png=$(left:.tif=.png)
right_png=$(right:.tif=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../../../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../../../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../../../code/$@ .

jaccard.py :
	-ln -s ../../../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/CT/specials/input/Makefile <==
SHELL = bash
.ONESHELL:

left=191146-1_distort_only_000445.png
right=191146-1_distort_only_000446.png
file_suffix=_ct-special_orig-num_445-446_

left_png=$(left:.tif=.png)
right_png=$(right:.tif=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../../../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../../../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../../../code/$@ .

jaccard.py :
	-ln -s ../../../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/CT/specials/input/Makefile_ <==
SHELL = bash
.ONESHELL:

left=rigid2_0_0300_def.tif
right=rigid2_0_0301_def.tif
file_suffix=_ct-sg_300-301_

left_png=$(left:.tif=.png)
right_png=$(right:.tif=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/CT/specials/surf-deform/Makefile <==
SHELL = bash
.ONESHELL:

left=warped2_3_0348.tiff
right=warped2_3_0349.tiff
file_suffix=_ct-special_surf-deform_348-349

left_png=$(left:.tif=.png)
right_png=$(right:.tif=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../../../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../../../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../../../code/$@ .

jaccard.py :
	-ln -s ../../../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/CT/specials/surf-deform/Makefile_ <==
SHELL = bash
.ONESHELL:

left=el_0099.png
right=el_0100.png
file_suffix=_ct-special_el_099-100

left_png=$(left:.tif=.png)
right_png=$(right:.tif=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../../../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../../../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../../../code/$@ .

jaccard.py :
	-ln -s ../../../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/EM/eval/em_distort-only/Makefile <==
SHELL = bash
.ONESHELL:

left=local_0500.png
right=local_0501.png
file_suffix=_em-LOCAL_ONLY_500-501_

left_png=$(left:.tiff=.png)
right_png=$(right:.tiff=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 150 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/EM/eval/em_el_prerigid_ol/Makefile <==
SHELL = bash
.ONESHELL:

left=el_0500.png
right=el_0501.png
file_suffix=_em-el_500-501_

left_png=$(left:.tiff=.png)
right_png=$(right:.tiff=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 150 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/EM/eval/em_funatomi/Makefile <==
SHELL = bash
.ONESHELL:

left=out1499.png
right=out1500.png
file_suffix=_em-funatomi_1499-1500__500-501_

left_png=$(left:.tiff=.png)
right_png=$(right:.tiff=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 150 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/EM/eval/em_orig-16bit/Makefile <==
SHELL = bash
.ONESHELL:

left=17-837b_bi3_rs+1+150_smROI_ROI01_adg_0500.tif
right=17-837b_bi3_rs+1+150_smROI_ROI01_adg_0501.tif
file_suffix=_em-FULL-ORIG-16bit__500-501_

left_png=$(left:.tif=.png)
right_png=$(right:.tif=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 5000 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/EM/eval/em_orig-norm/Makefile <==
SHELL = bash
.ONESHELL:

left=norm_0500.png.dump.png
right=norm_0501.png.dump.png
file_suffix=_em-orig-NORM-8bit_500-501_

left_png=$(left:.tiff=.png)
right_png=$(right:.tiff=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 150 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/EM/eval/em_sg/Makefile <==
SHELL = bash
.ONESHELL:

left=rigid2_0_0500_def.tif
right=rigid2_0_0501_def.tif
file_suffix=_em-sg_500-501_

left_png=$(left:.tif=.png)
right_png=$(right:.tif=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix)_100.txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard_CROP_$(file_suffix)_150.txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 150 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix)_100.txt jaccard_CROP_$(file_suffix)_150.txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/EM/eval/em_sift/Makefile <==
SHELL = bash
.ONESHELL:

left=rigid2_0_500.tiff
right=rigid2_0_501.tiff
file_suffix=_em-sift-rigid_500-501_

left_png=$(left:.tiff=.png)
right_png=$(right:.tiff=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 150 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/EM/eval/em_surf_dist-NORM/Makefile <==
SHELL = bash
.ONESHELL:

left=warped2_3_0500.tiff
right=warped2_3_0501.tiff
file_suffix=_em-surf-dist-norm_500-501_

left_png=$(left:.tiff=.png)
right_png=$(right:.tiff=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix)_100.txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard_CROP_$(file_suffix)_150.txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 150 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix)_100.txt jaccard_CROP_$(file_suffix)_150.txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/EM/eval/em_surf_rigid/Makefile <==
SHELL = bash
.ONESHELL:

left=rigid2_0_0500.tiff
right=rigid2_0_0501.tiff
file_suffix=_em-surf-rigid_500-501_

left_png=$(left:.tiff=.png)
right_png=$(right:.tiff=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix)_100.txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	/usr/local/Cellar/python\@3.8/3.8.6_1/bin/python3.8 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard_CROP_$(file_suffix)_150.txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	/usr/local/Cellar/python\@3.8/3.8.6_1/bin/python3.8 jaccard.py $(input_left_gray) $(input_right_gray) 150 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix)_100.txt jaccard_CROP_$(file_suffix)_150.txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/LS/eval/ls_el_prerigid_ol/Makefile <==
SHELL = bash
.ONESHELL:

left=el_0150.png
right=el_0151.png
file_suffix=_ls-el_150-151_

left_png=$(left:.tiff=.png)
right_png=$(right:.tiff=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/LS/eval/ls_funatomi/Makefile <==
SHELL = bash
.ONESHELL:

left=out0449.png
right=out0450.png
file_suffix=_ls-funatomi_449-450__150-151_

left_png=$(left:.tiff=.png)
right_png=$(right:.tiff=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/LS/eval/ls_local-only/Makefile <==
SHELL = bash
.ONESHELL:

left=local_0150.tiff
right=local_0151.tiff
file_suffix=_ls-local-only_150-151_

left_png=$(left:.tiff=.png)
right_png=$(right:.tiff=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/LS/eval/ls_norm/Makefile <==
SHELL = bash
.ONESHELL:

left=norm_0150.tiff
right=norm_0151.tiff
file_suffix=_ls-ground-norm_150-151_

left_png=$(left:.tiff=.png)
right_png=$(right:.tiff=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/LS/eval/ls_sg/Makefile <==
SHELL = bash
.ONESHELL:

left=rigid2_0_0150_def.tif
right=rigid2_0_0151_def.tif
file_suffix=_ls-sg_150-151_

left_png=$(left:.tif=.png)
right_png=$(right:.tif=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/LS/eval/ls_sift-rigid/Makefile <==
SHELL = bash
.ONESHELL:

left=rigid2_0_150.tiff
right=rigid2_0_151.tiff
file_suffix=_ls-sift-rigid_150-151_

left_png=$(left:.tiff=.png)
right_png=$(right:.tiff=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/LS/eval/ls_surf-deform_1e-2/Makefile <==
SHELL = bash
.ONESHELL:

left=warped2_3_0150.tiff
right=warped2_3_0151.tiff
file_suffix=_ls-surf-deform-1e-2_150-151_

left_png=$(left:.tiff=.png)
right_png=$(right:.tiff=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/LS/eval/ls_surf-deform_1e-3/Makefile <==
SHELL = bash
.ONESHELL:

left=warped2_3_0150.tiff
right=warped2_3_0151.tiff
file_suffix=_ls-surf-deform-1e-3_150-151_

left_png=$(left:.tiff=.png)
right_png=$(right:.tiff=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/LS/eval/ls_surf-deform_std/Makefile <==
SHELL = bash
.ONESHELL:

left=warped2_3_0150.tiff
right=warped2_3_0151.tiff
file_suffix=_ls-surf-deform-std_150-151_

left_png=$(left:.tiff=.png)
right_png=$(right:.tiff=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/LS/eval/ls_surf-rigid/Makefile <==
SHELL = bash
.ONESHELL:

left=rigid2_0_0150.tiff
right=rigid2_0_0151.tiff
file_suffix=_ls-surf-rigid_150-151_

left_png=$(left:.tiff=.png)
right_png=$(right:.tiff=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../code/$@ .

jaccard.py :
	-ln -s ../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/LS/specials/sg/Makefile <==
SHELL = bash
.ONESHELL:

left=rigid2_0_0161_def.tif
right=rigid2_0_0162_def.tif
file_suffix=_ls-special_sg_161-162

left_png=$(left:.tif=.png)
right_png=$(right:.tif=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../../../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../../../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../../../code/$@ .

jaccard.py :
	-ln -s ../../../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png


==> image/LS/specials/sg/Makefile_ <==
SHELL = bash
.ONESHELL:

left=warped2_3_0348.tiff
right=warped2_3_0349.tiff
file_suffix=_ct-special_surf-deform_348-349

left_png=$(left:.tif=.png)
right_png=$(right:.tif=.png)

color_left:=$(addprefix color_, $(left_png))
color_right:=$(addprefix color_, $(right_png))
gray_left:=$(addprefix gray_, $(left_png))
gray_right:=$(addprefix gray_, $(right_png))

input_left_color:=$(addprefix crop_, $(color_left))
input_right_color:=$(addprefix crop_, $(color_right))

input_left_gray:=$(addprefix crop_, $(gray_left))
input_right_gray:=$(addprefix crop_, $(gray_right))

# https://stackoverflow.com/a/2826068
# https://www.gnu.org/software/make/manual/html_node/Substitution-Refs.html
# https://stackoverflow.com/a/47676194
# http://www.imagemagick.org/discourse-server/viewtopic.php?t=34489
# https://stackoverflow.com/a/36148655

all : psnr ssim flow imshowpair jaccard

.PHONY: inputs

left.png : $(left)
	ln -s $< $@

right.png : $(right)
	ln -s $< $@

$(color_left) : $(left)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(color_right) : $(right)
	convert $< -colorspace RGB -define png:color-type=2 +repage $@

$(gray_left) : $(left)
	convert $< -colorspace Gray $@

$(gray_right) : $(right)
	convert $< -colorspace Gray $@

crop_% : %
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

$(input_left_color) : $(color_left)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

$(input_right_color) : $(color_right)
	convert $< -gravity center -crop 500x500+0+0 +repage -define png:color-type=2 -flatten $@

inputs : $(input_left_color) $(input_right_color)  $(input_left_gray) $(input_right_gray)  left.png right.png

crop_psnr_$(file_suffix).png : $(input_left_color) $(input_right_color)
	-identify $(input_left_color) $(input_right_color)
	-compare $(input_left_color) $(input_right_color) -compose Src -metric PSNR -fuzz 5% $@

psnr_file : crop_psnr_$(file_suffix).png

psnr_FULL_$(file_suffix).png : $(color_left) $(color_right)
	-identify $(color_left) $(color_right)
	-compare $(color_left) $(color_right) -compose Src -metric PSNR -fuzz 5% $@ 

crop_psnr_FULL_$(file_suffix).png : psnr_FULL_$(file_suffix).png

psnr_log : $(input_left_gray) $(input_right_gray)
	-compare  $(input_left_gray) $(input_right_gray) -compose Src -metric PSNR -fuzz 5% t.png 2> psnr_$(file_suffix).txt 1>&2
	rm -f t.png

psnr : psnr_file psnr_log

ssim_prepare :
	-ln -s ../../../code/ssim*m .

ssim_full : ssim_full_$(file_suffix).png

ssim_full_$(file_suffix).png : $(gray_left) $(gray_right) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFF 
	pkg load image;
	ssim_index(  "$(gray_left)" ,  "$(gray_right)" , "$@" );
	SSIMEOFF

crop_ssim_full_$(file_suffix).png : ssim_full_$(file_suffix).png
	convert $< -gravity center -crop 500x500+0+0 +repage -flatten $@

ssim_crop : crop_ssim_full_$(file_suffix).png

ssim_log : ssim_CROP_$(file_suffix).txt

ssim_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) ssim_prepare
	@echo "Please run me with GNU make!"
	-octave-cli <<- SSIMEOFC > $@
	pkg load image;
	ssim_index( "$(input_left_gray)" ,  "$(input_right_gray)", "ssim_CROP_$(file_suffix).png");
	SSIMEOFC
	-rm -f ssim_CROP_$(file_suffix).png

ssim : ssim_log ssim_crop ssim_prepare

show_flow.py :
	-ln -s ../../../code/$@ .

crop_flow_CROP_$(file_suffix).png : $(input_left_gray) $(input_right_gray) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(input_left_gray) $(input_right_gray) $@ ; \
	)

flow_FULL_$(file_suffix).png : $(gray_left) $(gray_right) show_flow.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 show_flow.py $(gray_left) $(gray_right) $@; \
	)

flow_crop_FULL : crop_flow_FULL_$(file_suffix).png

flow : crop_flow_CROP_$(file_suffix).png

imshowpair.py :
	-ln -s ../../../code/$@ .

jaccard.py :
	-ln -s ../../../code/$@ .

jaccard_CROP_$(file_suffix).txt : $(input_left_gray) $(input_right_gray) jaccard.py
	( \
	source ~/.virtualenvs/sklean/bin/activate; \
	python3 jaccard.py $(input_left_gray) $(input_right_gray) 100 > $@ \
	)

jaccard : jaccard_CROP_$(file_suffix).txt

crop_pair_$(file_suffix).png : $(input_left_gray) $(input_right_gray) imshowpair.py
	( \
	source ~/.virtualenvs/cv2/bin/activate; \
	python3 imshowpair.py $(input_left_gray) $(input_right_gray) $@ \
	)

imshowpair : crop_pair_$(file_suffix).png

